SoK: Microservice Architectures from a Dependability Perspective

The microservice software architecture leverages the idea of splitting large monolithic applications into multiple smaller services that interact using lightweight communication schemes. While the microservice architecture has proven its ability to support modern business applications, it also introduces new possible weak points in a system. Some scientific literature surveys have already addressed fault tolerance or security concerns but most of them lack analysis on the fault and vulnerability coverage that is introduced by microservice architectures. We explore the known faults and vulnerabilities that microservice architecture might suffer from, and the recent scientific literature that addresses them. We emphasize runtime detection and recovery mechanisms instead of offline prevention and mitigation mechanisms to limit the scope of this document.

==> Makefile <==
FILE=main.tex

default: ${FILE1}
	latexmk -pvc -pdf ${FILE}

# default: figures/bracha.pdf \
# 	figures/dolev.pdf \
# 	figures/transmissiongraph.pdf \
# 	figures/brachatransmission.pdf \
# 	figures/interfacesBrachaDolev.pdf \
# 	figures/interfacesBrachaCPA.pdf \
# 	figures/interfacesBrachaDolev_modified.pdf
# 	latexmk -pvc -pdf ${FILE1}

# figures/interfacesBrachaDolev.pdf: figures/interfacesBrachaDolev.svg
# 	(cd figures; inkscape --export-area-drawing --export-pdf=interfacesBrachaDolev.pdf interfacesBrachaDolev.svg)
# 	
# figures/interfacesBrachaCPA.pdf: figures/interfacesBrachaCPA.svg
# 	(cd figures; inkscape --export-area-drawing --export-pdf=interfacesBrachaCPA.pdf interfacesBrachaCPA.svg)
# 	
# figures/interfacesBrachaDolev_modified.pdf: figures/interfacesBrachaDolev_modified.svg
# 	(cd figures; inkscape --export-area-drawing --export-pdf=interfacesBrachaDolev_modified.pdf interfacesBrachaDolev_modified.svg)
# 
# figures/transmissiongraph.eps: figures/transmissiongraph.dia
# 	(cd figures; dia --export=transmissiongraph.eps transmissiongraph.dia)
# 
# figures/transmissiongraph.pdf: figures/transmissiongraph.eps
# 	(cd figures; epspdf  transmissiongraph.eps; pdfcrop transmissiongraph.pdf transmissiongraph.pdf)
# 
# figures/dolev.eps: figures/dolev.dia
# 	(cd figures; dia --export=dolev.eps dolev.dia)
# 
# figures/dolev.pdf: figures/dolev.eps
# 	(cd figures; epspdf  dolev.eps; pdfcrop dolev.pdf dolev.pdf)
# 
# figures/bracha.eps: figures/bracha.dia
# 	(cd figures; dia --export=bracha.eps bracha.dia)
# 
# figures/bracha.pdf: figures/bracha.eps
# 	(cd figures; epspdf  bracha.eps; pdfcrop bracha.pdf bracha.pdf)
# 
# figures/brachatransmission.eps: figures/brachatransmission.dia
# 	(cd figures; dia --export=brachatransmission.eps brachatransmission.dia)
# 
# figures/brachatransmission.pdf: figures/brachatransmission.eps
# 	(cd figures; epspdf  brachatransmission.eps; pdfcrop brachatransmission.pdf brachatransmission.pdf)

clean:
	rm -f *.aux *.bbl *.blg *.fdb_latexmk *.fls *.log *.out *.run.xml *.bcf *.dvi *.ps *.run.xml
	rm ${FILE}.pdf

cleanall:
	rm -f *.aux *.bbl *.blg *.fdb_latexmk *.fls *.log *.out *.bcf *.dvi *.run.xml *.tex~ Makefile~


